Linear Convergence in Hilbert's Projective Metric for Computing Augustin Information and a R\'{e}nyi Information Measure

Consider the problems of computing the Augustin information and a R\'{e}nyi information measure of statistical independence, previously explored by Lapidoth and Pfister (IEEE Information Theory Workshop, 2018) and Tomamichel and Hayashi (IEEE Trans. Inf. Theory, 64(2):1064--1082, 2018). Both quantities are defined as solutions to optimization problems and lack closed-form expressions. This paper analyzes two iterative algorithms: Augustin's fixed-point iteration for computing the Augustin information, and the algorithm by Kamatsuka et al. (arXiv:2404.10950) for the R\'{e}nyi information measure. Previously, it was only known that these algorithms converge asymptotically. We establish the linear convergence of Augustin's algorithm for the Augustin information of order $\alpha \in (1/2, 1) \cup (1, 3/2)$ and Kamatsuka et al.'s algorithm for the R\'{e}nyi information measure of order $\alpha \in [1/2, 1) \cup (1, \infty)$, using Hilbert's projective metric.

==> src/alternative_proofs.tex <==
% !TEX root = ../paper.tex

\section{An Alternative Proof of Theorem~\ref{thm:augustin_contraction}}\label{sec:alternative_proof}

Define $\tilde{\T}_x(q):={p_{Y|X}(\cdot|x)}^{\odot\alpha} \odot {q}^{\odot(1-\alpha)}$, which is the unnormalized version of $\T_x(q)$.
We will use the following two lemmas about $M$ and $\tilde{\T}_x$.
Their proofs are deferred to the next subsections.

\begin{lemma}\label{lem:mTx}
	Let $q, q'\in\Delta_n$ and $x\in[m]$.
	For $\alpha\in(0, 1)$, we have
	\begin{align*}
		M(\tilde{\T}_x(q)/\tilde{\T}_x(q')) &\leq M(q/q')^{ \abs{ 1-\alpha } }.
	\end{align*}
	For $\alpha\in(1, 2)$, we have
	\begin{align*}
		M(\tilde{\T}_x(q)/\tilde{\T}_x(q')) &\leq M(q'/q)^{ \abs{ 1-\alpha} }.
	\end{align*}
\end{lemma}


\begin{lemma}\label{lem:expectation}
	Let $u_X$ and $v_X$ be two random probability vectors in $\Delta_d$.
	We have
    \begin{equation*}
		M(\E_X[u_X] / \E_X[v_X]) \leq \sup_{x\in\mathcal{X}} M(u_x / v_x).
	\end{equation*}
\end{lemma}

\subsection{Proof of Theorem~\ref{thm:augustin_contraction}}
Recall that
\[
	\dH( \T(q), \T(q') )
	= \log(M(\T(q)/\T(q')) \cdot M(\T(q')/\T(q))).
\]
By Lemma \ref{lem:expectation}, we have
\[
    M(\T(q)/\T(q'))
    \leq\sup_x{ M(\T_x(q) / \T_x(q')) }
    =\sup_x{\frac{ \norm{ \tilde{\T}_x(q) }_1}{ \norm{ \tilde{\T}_x(q') }_1} M(\tilde{\T}_x(q)/\tilde{\T}_x(q'))},
\]
where the equality is due to the fact that $M(au/bv)=(a/b)M(u/v)$ for any $a, b>0$ and $u, v\in\R^d_+$.
To bound the ratio of the $1$-norms, notice that $\tilde{\T}_x(q) \leq M(\tilde{\T}_x(q)/\tilde{\T}_x(q')) \tilde{\T}_x(q')$, which implies
\[
	\frac{ \norm{ \tilde{\T}_x(q) }_1}{ \norm{ \tilde{\T}_x(q') }_1}
	\leq M(\tilde{\T}_x(q)/\tilde{\T}_x(q')).
\]
Therefore, we have
\begin{equation}\label{eq:mQQ'}
	M(\T(q)/\T(q')) \leq \sup_x M(\tilde{\T}_x(q)/\tilde{\T}_x(q'))^2.
\end{equation}
By symmetry, we also have
\begin{equation}\label{eq:mQ'Q}
	M(\T(q')/\T(q)) \leq \sup_x M(\tilde{\T}_x(q')/\tilde{\T}_x(q))^2.
\end{equation}


Next, by Lemma \ref{lem:mTx}, for $\alpha\in(0, 2) \setminus \{1\}$, we have either
\begin{align*}
    M(\tilde{\T}_x(q)/\tilde{\T}_x(q')) \leq M(q/q')^{ \abs{1-\alpha} }\quad\text{and}\quad 
    M(\tilde{\T}_x(q')/\tilde{\T}_x(q)) \leq M(q'/q)^{ \abs{1-\alpha} },
\end{align*}
or
\begin{align*}
    M(\tilde{\T}_x(q)/\tilde{\T}_x(q')) \leq M(q'/q)^{ \abs{1-\alpha} }\quad\text{and}\quad 
    M(\tilde{\T}_x(q')/\tilde{\T}_x(q)) \leq M(q/q')^{ \abs{1-\alpha} }.
\end{align*}
In either case, we have
\begin{align}\label{eq:2_abs}
	\sup_x M(\tilde{\T}_x(q)/\tilde{\T}_x(q'))^2 &\cdot
	\sup_x M(\tilde{\T}_x(q')/\tilde{\T}_x(q))^2 \\
    &\leq M(q/q')^{2 \abs{1-\alpha} } \cdot M(q'/q)^{2 \abs{1-\alpha} }.
\end{align}


Finally, combine the inequalities \eqref{eq:mQQ'}, \eqref{eq:mQ'Q}, and \eqref{eq:2_abs}, then we have
\begin{align*}
    \dH(\T(q), \T(q'))&=\log(M(\T(q)/\T(q')) M(\T(q')/\T(q)))\\
    &\leq \log(M(q/q')^{2|1-\alpha|} M(q'/q)^{2|1-\alpha|})\\
    &=2|1-\alpha|\dH(q, q').
\end{align*}
This completes the proof.


\subsection{Proof of Lemma~\ref{lem:mTx}}
We first prove the case when $\alpha\in(0,1)$.
	Since $\tilde{\T}_x$ is homogeneous of degree $(1-\alpha)$ and order-preserving, i.e.,
	\begin{align*}
		&\tilde{\T}_x(\mu q)=\mu^{1-\alpha}\tilde{\T}_x(q) \text{ for any } \mu>0\text{; and}\\
		&q\leq q' \implies \tilde{\T}_x(q)\leq \tilde{\T}_x(q'), 
	\end{align*}
	we have
	\begin{equation*}
		\tilde{\T}_x(q) \leq \tilde{\T}_x(M(q/q')q') = M(q/q')^{1-\alpha}\tilde{\T}_x(q'),
	\end{equation*}
	where the inequality is due to the fact that $q\leq M(q/q')q'$.
	According to the definition of $M$, this implies
	\begin{equation*}
		M(\tilde{\T}_x(q) / \tilde{\T}_x(q')) \leq M(q / q')^{1-\alpha}.
	\end{equation*}
	
%	\textbf{Case 2.} $\alpha\in(1, 2)$.
	Now, we prove the case when $\alpha\in(1,2)$.
	When $\alpha\in(1, 2)$, the operator $\tilde{\T}_x$ is still homogeneous of degree $(1-\alpha)$, but it becomes order-reversing, i.e.,
	\begin{equation*}
		q\leq q' \implies \tilde{\T}_x(q') \leq \tilde{\T}_x(q).
	\end{equation*}
	By a similar argument, we get
	\begin{equation*}
		\tilde{\T}_x(q') \geq \tilde{\T}_x(M(q'/q)q) = M(q'/q)^{1-\alpha}\tilde{\T}_x(q).
	\end{equation*}
	Thus, we have
	\begin{equation*}
		M(\tilde{\T}_x(q) / \tilde{\T}_x(q')) \leq M(q'/ q)^{\alpha-1}.
	\end{equation*}
	This completes the proof.


\subsection{Proof of Lemma~\ref{lem:expectation}}
    Let $M_0:=\sup_{x\in\mathcal{X}} M(u_x / v_x)$.
    We have
	\begin{equation*}
		M_0\E_X[v_X]=\E_X [M_0 v_X] \geq \E_X [M(u_X / v_X) v_X] \geq \E_X [u_X].
	\end{equation*}
	The lemma follows from the definition of $M$.

==> src/augustin_d_equals_2.tex <==
% !TEX root = ../paper.tex



\section{Augustin Information When $d=2$}
\label{sec:augustin_d_equals_2}

\subsection{Linear Convergence of Augustin's Fixed-Point Iteration}

Consider Augustin's fixed-point iteration \eqref{eq:cover}.
In the special case of $d=2$, the convergence results established in Section~\ref{sec:augustin} can be significantly improved, which we present in this section.
We follow the notations in Section~\ref{sec:augustin}.

The following theorem improves on Theorem~\ref{cor:augustin_linear_rate} when $d=2$.

\begin{theorem}\label{thm:augustin_contraction_d_equals_2}
Assume $d=2$.
For $\alpha\in[0,1)\cup(1,\infty)$, we have
\begin{equation}
	\dH(T_\alpha(x), T_\alpha(x'))\leq \gamma\cdot \dH(x, x'),\quad\forall x,x'\in\Delta([2]),
\end{equation}
where $\gamma:=|1-\alpha|$.
\end{theorem}

The proof of Theorem~\ref{thm:augustin_contraction_d_equals_2} parallels that of Theorem~\ref{thm:augustin_contraction} and is hence omitted.
The only difference is that we replace Lemma~\ref{lem:distance_of_expectation} with the following improvement when $d=2$.
The proof of Lemma~\ref{lem:distance_of_expectation_d_equals_2} is deferred to the next subsection.


\begin{lemma}\label{lem:distance_of_expectation_d_equals_2}
Assume $d=2$.
Let $X, Y: \Omega\to\Delta([2])$ be two random probability vectors.
We have
\[
	\dH\left( \E[ X ], \E[ Y ] \right)
	\leq \sup_{\omega\in\Omega} \dH( X(\omega), Y(\omega) ).
\]
\end{lemma}


Theorem~\ref{thm:augustin_contraction_d_equals_2} directly implies the following corollary, showing that when $d=2$, Augustin's fixed-point iteration converges linearly for all $\alpha\in(0,1)\cup(1,2)$.
Since the proof of Corollary~\ref{cor:augustin_linear_rate_d_equals_2} is the same as that of Corollary~\ref{cor:augustin_linear_rate}, it is omitted.

\begin{corollary}\label{cor:augustin_linear_rate_d_equals_2}
Assume $d=2$.
For $\alpha\in(0, 1)\cup(1, 2)$, let $x^\star$ be the minimizer of the optimization problem \eqref{eq:augustin_information} and $\{x_t\}$ be the iterates of Augustin's fixed-point iteration \eqref{eq:cover}.
We have
\[
	\dH(x_{t+1}, x^\star) \leq \gamma^t \cdot  \dH(x_1, x^\star),
\]
for all $t\in\N$, where $\gamma<1$ is defined in Theorem~\ref{thm:augustin_contraction_d_equals_2}.
\end{corollary}


\subsection{Proof of Lemma~\ref{lem:distance_of_expectation_d_equals_2}}

%Note that if there exists $\omega$ such that $\dH(X(\omega), Y(\omega)) = \infty$, then the lemma holds.
%In the following, we assume $\dH(X(\omega), Y(\omega)) < \infty$ for all $\omega$.

Let $D:=\sup_\omega\dH( X(\omega), Y(\omega) )$.
If $D = \infty$, then the lemma clearly holds.
We assume $D<\infty$ in the rest of the proof.

By Lemma~\ref{lem:hilberts_projective_metric}, Hilbert's projective metric between $x,y \in \Delta([2])$ can be written as
\[
	\dH( x, y ) := \max\left\{ \log \frac{x(1)(1-y(1))}{(1-x(1))y(1)}, \log \frac{(1-x(1))y(1)}{x(1)(1-y(1))} \right\}.
\]
We will use the following technical lemma, which involves the notion of quasi-convexity \citep{Greenberg1971}.
Its proof is postponed to the next subsection.

\begin{lemma}\label{lem:quasiconvex}
The function $\varphi:[0,1]^2\to\R\cup\{\infty\}$, defined as
\[
	\varphi( s, t ) := \max\left\{ \log \frac{s(1-t)}{(1-s)t}, \log \frac{(1-s)t}{s(1-t)} \right\},
\]
is jointly quasi-convex in $s$ and $t$, i.e., its lower level set
\[
	L_\alpha := \{ (s,t)\in[0,1]^2 : \varphi(s,t)\leq\alpha \}
\]
is convex for all $\alpha\in\R$.
\end{lemma}

For every $\omega\in\Omega$, since
\[
	\dH(X(\omega), Y(\omega))
	= \varphi( X(\omega)(1), Y(\omega)(1) ) \leq D,
\]
we have $( X(\omega)(1), Y(\omega)(1) ) \in L_D$.
By the quasi-convexity of $\varphi$, the set $L_D$ is convex, which implies $( \E_\omega[X(\omega)(1)], \E_\omega[Y(\omega)(1)] ) \in L_D$.
Hence,
\[
	\dH( \E[X], \E[Y] )
	=
	\varphi( \E_\omega[X(\omega)(1)], \E_\omega[Y(\omega)(1)] )
	\leq D.
\]
This completes the proof.


\subsection{Proof of Lemma~\ref{lem:quasiconvex}}
When $\alpha<0$, since $\varphi(s,t)$ is a metric, the set $L_\alpha$ is empty, which is convex by the definition.
Now assume $\alpha\geq 0$.
First, we write $L_\alpha$ as the intersection of two sets:
\begin{multline*}
	L_\alpha = \left\{ (s,t)\in[0,1]^2 : \log \frac{s(1-t)}{(1-s)t} \leq \alpha \right\} \\
	\cap \left\{ (s,t)\in[0,1]^2 : \log \frac{(1-s)t}{s(1-t)} \leq \alpha \right\}.
\end{multline*}
By some algebraic manipulations, we have
\[
	L_\alpha = \left\{ (s,t)\in[0,1]^2 : t \geq g_\alpha(s) \right\}
	\cap \left\{ (s,t)\in[0,1]^2 : t \leq g_{-\alpha}(s) \right\},
\]
where
\[
	g_\beta(s) := \frac{s}{s+\eu^{\beta}(1-s)}.
\]
In other words, $L_\alpha$ is the intersection of the epigraph of $g_\alpha$ and the subgraph of $g_{-\alpha}$.
To prove the convexity of $L_\alpha$, it suffices to show that $g_{\alpha}$ is convex on $[0,1]$ and $g_{-\alpha}$ is concave on $[0,1]$.
Then, since the epigraph of $g$ is convex and the subgraph of $h$ is convex, their intersection $L_\alpha$ will be convex.

By a direct calculation, we have
\[
	g_\beta''(s) = \frac{2(\eu^{\beta}-1)}{( s+\eu^{\beta}(1-s) )^3}.
\]
Since $\alpha\geq 0$, we have $g_{\alpha}''(s)\geq 0$ and $g_{-\alpha}''(s)\leq 0$ for all $s\in[0,1]$, implying that $g_{\alpha}$ is convex on $[0,1]$ and $g_{-\alpha}$ is concave on $[0,1]$.
The lemma follows.





==> src/introduction.tex <==
% !TEX root = ../paper.tex

\section{Introduction}

Several information quantities are defined by optimization problems and do not have closed-form expressions.
It is important to design optimization methods that can compute these quantities efficiently.
This work analyzes two optimization methods for computing the Augustin information \citep{Augustin1978,Csiszar1995} and a R\'{e}nyi information measure \citep{Lapidoth2019,Tomamichel2018}, respectively.


We now define the Augustin information.
Let $X$ and $Y$ be two random variables taking values in two finite sets $\mathcal{X}$ and $\mathcal{Y}$, respectively.
Let $p_{XY}$ be their joint probability distribution and $p_{Y|X}$ be the conditional distribution.
For $\alpha\in(0,\infty)\setminus\{1\}$, the order-$\alpha$ Augustin information is defined as
\begin{equation}\label{eq:augustin_information}
	I_\alpha (X; Y)
	:= \min_{q}\E_X\left[ D_\alpha( p_{Y|X}(\cdot|X) \parallel q ) \right],
\end{equation}
where the minimization is taken over all probability distributions on $\mathcal{Y}$, and
\[
	D_\alpha(p \parallel q):=\frac{1}{\alpha - 1}\log\sum_{z \in \mathcal{Z}} p(z)^{\alpha} q(z)^{1-\alpha}
\]
is the order-$\alpha$ R\'{e}nyi divergence between two probability distributions $p$ and $q$ on a finite set $\mathcal{Z}$.
%The Augustin information has wide applications in information theory.
The Augustin information characterizes the cutoff rate \citep{Csiszar1995}, the strong converse exponent \citep{Arimoto1973}, and the error exponent for constant composition codes \citep{Csiszar2011} in the channel coding problem.
For other applications, readers are referred to, e.g., the works of \citet{Nakiboglu2019} and \citet{Wang2024}, and references therein.
%We refer readers to our work \citep{Wang2024} for a comprehensive list of applications and references therein.


Following the above notations, for $\alpha\in(0,\infty)\setminus\{1\}$, the order-$\alpha$ R\'{e}nyi information measure is defined as
\begin{equation}\label{eq:renyi_information_measure}
	J_\alpha (X;Y)
	:= \min_{q_X, q_Y} D_\alpha( p_{XY} \parallel q_X \otimes q_Y ),
\end{equation}
where the minimization is over all probability distributions on $\mathcal{X}$ and $\mathcal{Y}$.
The R\'{e}nyi information measure appears in the error exponent and the strong converse exponent of the type-I error in a hypothesis testing problem, where given a sequence of i.i.d.~pairs of random variables $\{ (X_t,Y_t) \}$, we decide whether they come from some product distribution or not \citep{Lapidoth2019,Lapidoth2018,Tomamichel2018}.


%For $\alpha\in(0,\infty)\setminus\{1\}$, the optimization problem \eqref{eq:augustin_information} defining the Augustin information is convex \citep{Erven2014}.
%For $\alpha\in[1/2,\infty) \setminus \{1\}$, the optimization problem \eqref{eq:renyi_information_measure} defining the R\'{e}nyi information measure is also convex \citep{Lapidoth2019}.
%However, these two information quantities are not easy to compute.
%One may apply standard optimization algorithms, such as projected gradient descent (PGD) or interior point methods (IPMs), to compute the two information quantities.
%For example, projected gradient descent (PGD) does not directly apply because the objective functions in both problems violate standard assumptions for convergence, such as Lipschitz continuity and Lipschitz continuous gradients \citep{Nesterov2018}.
%Furthermore, projection onto the set of probability distributions can result in a distribution without full support.
%This can cause PGD to ``stall''; see \citet{You2022} for a detailed discussion.
%It is unclear how to choose appropriate step sizes so that PGD converges to the optimal value.
%Although we can apply interior point methods to solve the optimization problems, IPMs are computationally expensive and are not scalable with respect to the sizes of $\mathcal{X}$ and $\mathcal{Y}$.



Several existing optimization methods can be used to compute the two information quantities, which we review in Section~\ref{sec:related_work}.
In short, all of them achieve sublinear convergence rates at best.
We are particularly interested in a fixed-point iteration proposed by \citet{Augustin1978} for computing the Augustin information, which has been shown to converge asymptotically for $\alpha\in(0,1)$ \citep{Nakiboglu2019}.
We are also interested in an alternating minimization method proposed by \citet{Kamatsuka2024} for computing the R\'{e}nyi information measure, which has been proved to exhibit asymptotic convergence for $\alpha\in(0,\infty)\setminus\{1\}$.
The update rules of these two methods consist of entry-wise products and entry-wise powers of vectors.
This structure suggests that Hilbert's projective metric, which we introduce in the next paragraph, can be an effective tool for analyzing these two methods.


Hilbert's projective metric over the positive orthant is defined as\footnote{The general definition is given in Section~\ref{sec:preliminaries}.}
\begin{equation}
	\dH(x,y) := \log\max_{1\leq i,j\leq d}\frac{x(i)y(j)}{y(i)x(j)},
	\quad\forall x,y\in [0,\infty)^d.
\end{equation}
It enjoys a few useful properties for handling entry-wise operations.
For example, it holds that $\dH(x^{\odot r},y^{\odot r}) \leq \abs{r}\dH(x,y)$ for any exponent $r\in\R$, where $x^{\odot r}$ denotes the entry-wise power.
In the optimization literature, Hilbert's projective metric has been used to analyze Sinkhorn's algorithm for the matrix scaling problem \citep{Sinkhorn1964,Peyre2019}:
\citet{Franklin1989} showed that the iterates of Sinkhorn's algorithm converge linearly to the optimal point with respect to Hilbert's projective metric.


%Several methods can be used to solve the optimization problems \eqref{eq:augustin_information} and \eqref{eq:renyi_information_measure}.
%%, and they are guaranteed to converge asymptotically or to converge at a sublinear rate.
%For the Augustin information, a fixed-point iteration \citep{Augustin1978,Nakiboglu2019} and an alternating minimization method \citep{Karakos2008} converge asymptotically for $\alpha\in(0,1)$.
%We find that these two methods are, in fact, identical.\footnote{Each iteration of the alternating minimization method \citep{Karakos2008} consists of two steps.
%Combining these two steps yields the exact fixed-point iteration \citep{Augustin1978,Nakiboglu2019}.}
%Another alternating minimization method \citep{Kamatsuka2024} converges at a sublinear rate for $\alpha\in(1,\infty)$.\footnote{\citet{Kamatsuka2024} only claimed an asymptotic convergence guarantee in their paper.
%We find that their Lemma~2 implies a convergence rate of $O(1/t)$.}
%For any $\alpha\in(0,\infty)\setminus\{1\}$, entropic mirror descent with Armijo line search \citep{Li2018} and with Polyak step size \citep{You2022} both converge asymptotically, while Riemannian gradient descent with the Poincar\'{e} metric \citep{Wang2024} converges at a sublinear rate.
%For the R\'{e}nyi information measure, entropic mirror descent with Armijo line search \citep{Li2018} and an alternating minimization method \citep{Kamatsuka2024} converge asymptotically for $\alpha\in[1/2,\infty)\setminus\{1\}$.
%For $\alpha\in(0,1/2)$, the optimization problem can be non-convex \citep{Lapidoth2019}, and we are not aware of any method that provably solves the problem.


%Sublinear rates are unsatisfactory if we want high-accuracy estimates of the two information quantities \eqref{eq:augustin_information} and \eqref{eq:renyi_information_measure}.
%To compute one more correct digit, we need to spend an effort comparable to what we have put in so far \citep{Nesterov2018}.
%Therefore, we may aim to achieve faster convergence guarantee, such as linear convergence rates.
%Standard linear convergence results of projected gradient descent require the objective function to have a Lipschitz continuous gradient and to be strongly convex \citep{Nesterov2018}.
%However, \citet{You2022} and \citet{Wang2024} have already shown the lack of Lipschitz continuous gradients of the objective functions in the optimization problems \eqref{eq:augustin_information} and \eqref{eq:renyi_information_measure}.


%To design linearly convergent methods, we turn our attention to the fixed-point iteration \citep{Augustin1978,Karakos2008,Nakiboglu2019} for computing the Augustin information and the alternating minimization method \citep{Kamatsuka2024} for computing the R\'{e}nyi information measure.
%These two methods are similar to Sinkhorn's algorithm \citep{Sinkhorn1964,Peyre2019} for solving the matrix-scaling problem:
%all three methods use entry-wise operations, and their optimization problems all involve logarithmic functions.
%Since Sinkhorn's algorithm has been proved to converge linearly with respect to Hilbert's projective metric \citep{Franklin1989}, we ask whether the other two methods also have linear convergence.


%\deleted{
%In this work, we show that the answer is yes for a wide range of $\alpha$, thereby providing the first linearly convergent methods for computing the two information quantities, respectively.
%We summarize our results below.}


In this work, we use Hilbert's projective metric to analyze the fixed-point iteration \citep{Augustin1978,Nakiboglu2019} and the alternating minimization method \citep{Kamatsuka2024}.
We summarize our results below.

\begin{itemize}
\item For the Augustin information \eqref{eq:augustin_information} of order $\alpha\in(1/2,3/2)\setminus\{1\}$, the fixed-point iteration \citep{Augustin1978} converges at a rate of $O((2\abs{1-\alpha})^t)$ with respect to Hilbert's projective metric.
This improves on the previous asymptotic convergence guarantee \citep{Nakiboglu2019} for $\alpha\in(1/2,1)$ and extends the range of convergence to include $\alpha\in(1,3/2)$.

\item For the R\'{e}nyi information measure \eqref{eq:renyi_information_measure} of order $\alpha\in(1/2,\infty)\setminus\{1\}$, the alternating minimization method \citep{Kamatsuka2024} converges at a rate of $O(\abs{1-1/\alpha}^{2t})$ with respect to Hilbert's projective metric.
When $\alpha=1/2$, this method also converges linearly if $p_{XY}$ has full support.
This improves on the previous asymptotic convergence guarantee \citep{Kamatsuka2024}.
\end{itemize}

%\deleted{
%Our convergence analyses rely on properties of Hilbert's projective metric.
%Despite their simplicity, our analyses yield better convergence rates compared to existing ones.
%Our techniques can potentially be used for other related problems, such as computing the log-optimal portfolio \citep{Cover1984}.
%We will discuss this problem in Section~\ref{sec:discussions}.
%}

Compared to existing works, we establish the first linear convergence rates for computing the two information quantities, respectively.
Our analyses are simple yet yield significantly better convergence rates, demonstrating the importance of choosing suitable metrics when analyzing optimization methods.
Our techniques can potentially be used for other related problems, such as computing the log-optimal portfolio \citep{Cover1984}.
We discuss future directions in Section~\ref{sec:discussions}.
%While we only consider the problems of computing the Augustin information and the R\'{e}nyi information measure, 

%Our techniques can potentially be used for other related problems.
%We discuss potential applications of our techniques to other problems in Section~\ref{sec:discussions}.
%This demonstrates the importance of choosing suitable metrics when analyzing optimization methods.
%Our techniques can potentially be used for other related problems.

\paragraph{Notations}
Denote $\R_+ := [0,\infty)$ and $\R_{++} := (0,\infty)$.
Denote $[n] := \{ 1, 2,\ldots, n\}$ for $n\in\N$.
Denote by $\Delta_d:= \{ x\in\R_+^d \mid \norm{x}_1 = 1\}$ the probability simplex.
For $v\in\R^d$, denote by $v(i)$ its $i$-th entry.
Similarly, for $A\in\R^{m\times n}$, denote by $M(i,j)$ its $(i,j)$-th entry.
For $A,B\in\R^{m\times n}$ and $r\in\R$, denote by $A\odot B$ and $A^{\odot r}$ the entry-wise multiplication and entry-wise power, respectively.
For $S\subseteq\R^d$, denote by $\ri S$ its relative interior.
We adopt the convention that $0/0=1$, $\infty\cdot\infty=\infty$, $a\cdot\infty=\infty$ for any $a>0$, and $\log\infty=\infty$.




==> src/log_optimal_portfolio.tex <==
% !TEX root = ../paper.tex

\section{The Log-Optimal Portfolio}\label{sec:log_optimal_portfolio}

Consider the problem of computing the log-optimal portfolio \citep{Cover1984}, defined as

\begin{equation}\label{eq:log_optimal_portfolio}
	\min_{x\in\Delta_d} f(x),\quad f(x) := \E_a\left[ -\log\braket{ a, x} \right],
\end{equation}
where $a$ is a random vector taking values in $\R_+^d\setminus\{0\}$ and $d\geq 2$.


In this section, we analyze the fixed-point iteration of \citet{Cover1984} for solving the optimization problem \eqref{eq:log_optimal_portfolio}.
This fixed-point iteration has been proved to converge sublinearly \citep{Iusem1992,Lin2021}, while we observe that it often converges linearly.
We provide two results to complement our observations.
First, we show that the fixed-point iteration is \emph{not} a contraction with respect to Hilbert's projective metric.
Second, we show that it achieves a linear convergence rate asymptotically when $d=2$.


\subsection{The Fixed-Point Iteration}
Define the operator $S(x) := x\odot(-\nabla f(x))$ and consider the following fixed-point iteration:
\begin{enumerate}
    \item Initialize $x_1\in\Delta_d$.
    \item For all $t\in\N$, compute $x_{t+1} = S(x_t)$.
\end{enumerate}
Expand the definition of $\nabla f(x)$, and we get
\[
	S(x) = \E_a\left[ \frac{a\odot x}{\braket{a,x}} \right].
\]
Observe that the operator $S$ is the limit of the operator $T$ \eqref{eq:operator_augustin} for computing the Augustin information when $\alpha$ approaches $0$.
This fixed-point iteration is motivated by the following observation \citep{Cover1984}.
\begin{lemma}[\citet{Cover1984}]
If $x^\star$ is a minimizer of the optimization problem \eqref{eq:log_optimal_portfolio}, then $x^\star = S(x^\star)$.
In particular, if $x^\star\in\ri\Delta_d$, then $\nabla_i f(x^\star) = -1$ for all $i\in[d]$.
\end{lemma}



\subsection{Non-Contractivity of the Fixed-Point Iteration}
The following theorem shows that the Lipschitz constant of the operator $S$ with respect to Hilbert's projective metric is at least $1$.
Thus, it is not a contraction.
The proof is inspired by a proof of Birkhoff's contraction theorem \citep{Cavazos-Cadena2003} and is deferred to Section~\ref{sec:non_contractivity_proof}.


\begin{theorem}\label{thm:non_contractivity}
We have
\[
	\sup_{x,y\in\ri\Delta_d} \frac{ \dH(S(x), S(y)) }{ \dH(x, y) } \geq 1.
\]
\end{theorem}



\subsection{Asymptotic Linear Convergence of the Fixed-Point Iteration}

The following theorem provides an upper bound on the contraction ratio of the operator $S$ with respect to Hilbert's projective metric.
The proof is technical and deferred to Section~\ref{sec:log_optimal_portfolio_contraction_ratio}


\begin{theorem}\label{thm:log_optimal_portfolio_contraction_ratio}
Assume $x^\star\in\ri\Delta_d$.
We have
\[
	\limsup_{x\to x^\star}\frac{ \dH(Sx, x^\star) }{ \dH(x,x^\star) } \leq L:=\max_{i\neq j} \nabla^2_{ij}f(x^\star).
\]
\end{theorem}


The following corollary shows that when $d=2$ and $a(1)/a(2)$ is not a constant, the fixed-point iteration converges at a linear rate asymptotically.
The proof is deferred to Section~\ref{sec:log_optimal_portfolio_d_2}.

\begin{corollary}\label{cor:log_optimal_portfolio_d_2}

Assume $d=2$, $x^\star\in\ri\Delta_d$, and $a(1)/a(2)$ is not a constant.
Let $\{ x_t \}$ be the iterates of the fixed-point iteration.
Then, we have $L=\nabla^2_{12}f(x^\star)<1$.
This implies for any $L'\in(L,1)$, there exists $T\in\N$ such that
\[
	\dH( x_{t+1}, x^\star ) \leq L'\cdot \dH(x_t, x^\star)
\]
for all $t\geq T$.
\end{corollary}



\subsection{Proof of Theorem~\ref{thm:non_contractivity}}\label{sec:non_contractivity_proof}

Since $\dH$ is a projective metric, we have
\[
	\sup_{x,y\in\R_{++}^d} \frac{ \dH(S(x), S(y)) }{ \dH(x, y) } = \sup_{x,y\in\ri\Delta_d} \frac{ \dH(S(x), S(y)) }{ \dH(x, y) }.
\]
For $\varepsilon>0$ and $t\geq 0$, let $x_t = (\eu^t, \varepsilon, \ldots, \varepsilon)^\top$.
It can be checked that $\dH(x_t,x_0)=t$.
We will show that
\begin{equation}\label{eq:double_limit}
	\liminf_{\varepsilon\to 0^+}\lim_{t\to 0^+}\frac{ \dH(S(x_t), S(x_0)) }{ \dH(x_t, x_0) } \geq 1.
\end{equation}
Suppose \eqref{eq:double_limit} holds.
Since $x_t,x_0\in\R_{++}^d$ for every $\varepsilon>0$, we have
\[
	\sup_{x,y\in\R_{++}^d} \frac{ \dH(S(x), S(y)) }{ \dH(x, y) }
	\geq \liminf_{\varepsilon\to 0^+}\lim_{t\to 0^+}\frac{ \dH(S(x_t), S(x_0)) }{ \dH(x_t, x_0) } \geq 1,
\]
and the proof is complete.


Now we prove \eqref{eq:double_limit}.
First, write
\[
	\dH(S(x_t), S(x_0))
	= \log \frac{ S(x_t)(1) S(x_0)(2) }{ S(x_0)(1) S(x_t)(2) }
	= \phi(t) - \phi(0),
\]
where
\[
	\phi(t) = \log S(x_t)(1) - \log S(x_t)(2)
	= t + \log\E\left[ \frac{a(1)}{\braket{a,x_t}}\right] - \log\E\left[ \frac{a(2)}{\braket{a,x_t}} \right] - \log\varepsilon.
\]
We have
\[
	\lim_{\varepsilon\to 0^+}\lim_{t\to 0^+} \frac{ \dH(S(x_t), S(x_0)) }{ \dH(x_t, x_0) }
	=
	\lim_{\varepsilon\to 0^+}\lim_{t\to 0^+} \frac{ \phi(t) - \phi(0) }{ t }
	= \lim_{\varepsilon\to 0^+}\phi'(0).
\]
A direct calculation gives
\[
	\phi'(0) = 1 + \frac{ \E\left[ \frac{a(1)a(2)}{ \braket{a,x_0}^2 } \right] }{ \E\left[ \frac{a(2)}{ \braket{a,x_0} } \right] }
	- \frac{ \E\left[ \frac{a(1)^2}{ \braket{a,x_0}^2 } \right] }{ \E\left[ \frac{a(1)}{ \braket{a,x_0} } \right] }.
\]
By Lemma~\ref{lem:fraction_of_sums}, we have
\[
	\phi'(0) \geq 1 + \min_a \frac{a(1)}{ \braket{a,x_0} } - \max_a \frac{a(1)}{\braket{a,x_0}}.
\]
Finally, as $\varepsilon\to0$, we have $\braket{a,x_0}\to a(1)$ and
\[
	\liminf_{\varepsilon\to 0^+}\phi'(0)
	\geq 1 + 1 - 1
	= 1.
\]
This proves \eqref{eq:double_limit}.


\subsection{Proof of Theorem~\ref{thm:log_optimal_portfolio_contraction_ratio}}\label{sec:log_optimal_portfolio_contraction_ratio}


Without loss of generality, we assume
\begin{equation} \label{eq:ratio_order}
	\frac{x^\star(2)}{x(2)} \leq \frac{x^\star(i)}{x(i)} \leq \frac{x^\star(1)}{x(1)}, \quad\forall i\in [d].
\end{equation}
Then, we have $M(x/x^\star) = x(2)/x^\star(2)$, $M(x^\star/x) = x^\star(1)/x(1)$.
Write
\[ \begin{split}
	&\dH( x,x^\star ) = \log \frac{x(2)x^\star(1)}{x^\star(2)x(1)} =  (E_2-E_1)(x^\star) - (E_2-E_1)(x),\\
	&\dH(S(x), S(x^\star)) = \max_{i\neq j} \log \frac{ S(x)(i)S(x^\star)(j) }{ S(x^\star)(i)S(x)(j) }
	=  \max_{i\neq j} ( \phi_{ij}(x^\star) - \phi_{ij}(x)),
\end{split}
\]
where
\[\begin{split}
	E_i(x) &:= -\log x(i),\\
	R_i(x) &:= \log (-\nabla f_i(x)),\\
	\phi_{ij}(x) &:= \log S(x)(j) - \log S(x)(i) = (R_j - R_i + E_i- E_j)(x).
\end{split}
\]
We have
\[
	\frac{ \dH(S(x), S(x^\star)) }{ \dH( x,x^\star )  }
	= \max_{i\neq j}\frac{ \phi_{ij}(x^\star) - \phi_{ij}(x) }{ (E_2-E_1)(x^\star) - (E_2-E_1)(x) }.
\]


We first simplify the ratio inside the maximum.
Fix any distinct $i$ and $j$.
By Cauchy's mean value theorem, there exists a point $y = (1-t)x + tx^\star$ for some $t\in[0,1]$ such that
\[
	\frac{ \phi_{ij}(x) - \phi_{ij}(x^\star) }{ \psi_{12}(x) - \psi_{12}(x^\star) }
	= \frac{ \D\phi_{ij}(y)[x^\star-x] }{ \D(E_2-E_1)(y)[x^\star-x] }.
\]
Since $x^\star-y = (1-t)(x^\star-x)$, the above ratio can be written as
\[
	\frac{ \phi_{ij}(x) - \phi_{ij}(x^\star) }{ \psi_{12}(x) - \psi_{12}(x^\star) }
	= \frac{ \D\phi_{ij}(y)[x^\star-y] }{ \D(E_2-E_1)(y)[x^\star-y] }.
\]
According to Lemma~2 of \citet{Lin2021}, the function $R_i(x)$ is convex.
It is not hard to verify that both $E_i(x)$ and $R_i(x)$ are $1$-log-homogeneous barriers \citep{Nesterov1994}.
By Proposition~2.3.4 of \citet{Nesterov1994}, we have \[
	\D E_i(y)[y] = \D R_i(y)[y] = -1,\quad\forall i\in[d],
\]
which implies
%\[\begin{split}
%	\D(E_j-E_i)(y)[y-x^\star] &= -\D(E_j-E_i)(y)[x^\star], \\
%	\D\phi_{ij}(y)[y-x^\star] &= -\D\phi_{ij}(y)[x^\star].
%\end{split}
%\]
%Therefore, we have
\begin{equation}\label{eq:simplified_ratio}
	\frac{ \phi_{ij}(x) - \phi_{ij}(x^\star) }{ \psi_{12}(x) - \psi_{12}(x^\star) }
	= \frac{ \D\phi_{ij}(y)[x^\star] }{ \D(E_2-E_1)(y)[x^\star] }.
\end{equation}


To upper bound the ratio \eqref{eq:simplified_ratio}, we will use the following three ingredients.

\begin{enumerate}[label=(\roman*)]
\item For any $\delta>0$, by the continuity of $\nabla^2_{ij}f(x)$ and $-\nabla_i f(x)$, we assume $x$ is close enough to $x^\star$ so that
\begin{equation} \label{eq:}
	\nabla^2_{ij} f(y) \leq \nabla^2_{ij} f(x^\star) + \delta \leq L + \delta
	\quad\text{and}\quad
	\frac{1}{\nabla_i f(y)} \leq 1+\delta,
\end{equation}
for all distinct $i$ and $j$.

\item By the assumption \eqref{eq:ratio_order}, we have
\[
	\D E_1(y)[x^\star] \leq \D E_i(y)[x^\star] \leq \D E_2(y)[x^\star] ,\quad\forall i\in[d].
\]

\item Since $R_i$ is an $1$-log-homogenous barrier, we have
\[
	\D R_i(y)[x] = \D R_i(y)[x] + \D E_i(y)[x]\cdot \left( \D R_i(y)[y] + 1 \right).
\]
Expanding the right hand side gives
\[
	\D R_i(y)[x]
	= \D E_i(y)[x] + \sum_{k=1}^d y(k)\left( \frac{\nabla^2_{ik}f(y)}{-\nabla_k f(y)} \right) \D(E_k-E_i)(y)[x].
\]
\end{enumerate}


Recall that $\D\phi_{ij} = \D(R_j - E_j - R_i + E_i)$.
Applying the three items above, we have
\[
\begin{split}
	&\D (R_j-E_j)(y)[x^\star]
	\leq (L+\delta)(1+\delta) \sum_{k=1}^d y(k)\D(E_k-E_1)(y)[x^\star], \\
	&\D (-R_i+E_i)(y)[x^\star]
	\leq (L+\delta)(1+\delta) \sum_{k=1}^d y(k)\D(E_2-E_k)(y)[x^\star].
\end{split}
\]
Sum the above two inequalities, then we obtain
\[\begin{split}
	\D\phi_{ij}(y)[x^\star]
	&\leq (L+\delta)(1+\delta)\sum_{k=1}^d y(k) \D(E_2-E_1)(y)[x^\star]  \\
	&= (L+\delta)(1+\delta)\D(E_2-E_1)(y)[x^\star].
\end{split}
\]
Therefore, we have
\[
	\eqref{eq:simplified_ratio} \leq (L+\delta)(1+\delta).
\]


Finally, we conclude that for any $\delta>0$, we have
\[
	\frac{ \dH(S(x), S(x^\star)) }{ \dH( x,x^\star )  }
 \leq (L+\delta)(1+\delta),
\]
for any $x$ sufficiently close to $x^\star$.
This proves the theorem.



\subsection{Proof of Corollary~\ref{cor:log_optimal_portfolio_d_2}}
\label{sec:log_optimal_portfolio_d_2}

Expand the definition of $L=\nabla^2_{12}f(x)$, and we get
\[
	L = \E_a\left[ \frac{ a(1)a(2) }{ (a(1)x^\star(1) + a(2)x^\star(2))^2 }  \right]
	= \E_a\left[ g_1\left(\frac{a(1)}{a(2)}\right)g_2\left(\frac{a(1)}{a(2)}\right) \right],
\]
where 
\[
	g_1(t) = \frac{t}{tx^\star(1)+x^\star(2)},\quad
	g_2(t) = \frac{1}{tx^\star(1)+x^\star(2)}.
\]


Since $a(1)/a(2)$ is not a constant, $g_1$ is strictly increasing, and $g_2$ is strictly decreasing, by the FKG inequality \citep[Section~2.2]{Grimmett1999}, we have
\[
\begin{split}
	L &< \E_a\left[ g_1\left(\frac{a(1)}{a(2)}\right) \right]\cdot \E_a\left[ g_2\left(\frac{a(1)}{a(2)}\right) \right] = (-\nabla_1 f(x^\star)) \cdot (-\nabla_2 f(x^\star)) = 1.
\end{split}
\]
This completes the proof.

